An elementary introduction to information geometry

In this survey, we describe the fundamental differential-geometric structures of information manifolds, state the fundamental theorem of information geometry, and illustrate some use cases of these information manifolds in information sciences. The exposition is self-contained by concisely introducing the necessary concepts of differential geometry, but proofs are omitted for brevity.

==> quizz.tex <==
\begin{itemize}
	\item Can an IG manifold  be defined without a dissimilarity?
	
	\item Can a powered divergence $D^\beta$   be turned int a metric distance?
	
	\item Can a Riemannian distance be a divergence?
	
	\item Given two conjugate connections,  can we always build an $\alpha$-family of divergence?
	
	
\end{itemize}

==> surplus.tex <==

We outline this tutorial as follows: 

We explain the core information-geometric structure in \S\ref{sec:igstructure} that relies on  two independent differential-geometric concepts: (1) the metric tensors $g$ and (2) the affine connections $\nabla$, explained in \S\label{sec:dg}. 
An information-geometric manifold $M$ is equipped with 
a pair of conjugate affine connections~\cite{ConjConnection-1991} $\nabla$ and $\nabla^*$ (usually called 
dual connections\footnote{Despite the fact that there is a distinction between conjugate connections and dual connections in affine differential geometry~\cite{ConjConnection-1991}.} in information geometry) that is coupled to a metric tensor $g$ yielding the structure denoted by $(M,g,\nabla,\nabla^*)$ (\S\label{sec:igmfd}). 
The coupling of conjugate connections to the metric tensor implies that the dual parallel transport is metric compatible.
This  dualistic structure $(M,g,\nabla,\nabla^*)$ gives rise to a {\em statistical manifold}\footnote{This calling is a bit awkward since it can be applied in non-statistical contexts. However, it was shown recently that statistical manifold structures can be realized by statistical models~\cite{smsm-2006}.} structure $(M,g,C)$  (\S\label{sec:igstatmfd}) where $C$ is a totally symmetric cubic tensor~\cite{Lauritzen-1987}. From the derived structure $(M,g,C)$, we can always derive a one-parametric family of information-geometric manifolds 
$(M,g,\nabla^\alpha,(\nabla^\alpha)^*=\nabla^{-\alpha})$ (with $\alpha\in\bbR$). 
We report the fundamental theorem of information geometry that states that if $M$ has constant curvature with respect to $\nabla^\alpha$ then it has the same constant curvature for the conjugate connection $\nabla^{-\alpha}$ (\S\label{sec:igstatmfd}).
The first conjugate connections reported in information geometry was the {\em expectation connection} $\idxSup{e}\nabla$ and the {\em mixture connection} $\idxSup{m}\nabla=\idxSup{e}\nabla^*$ that defines the {\em expected geometry}, and the family of expected $\alpha$-connections via the cubic tensor $C$, called the {\em skewness tensor} in this context.
Notice that at this point there is no associated distance to these information-geometric manifolds $(M,g,\nabla,\nabla^*)$ or $(M,g,C)$.
However, we can  build an information-geometric structure $(M,g,\idxDiv{D}\nabla,\idxDiv{D^*}\nabla=\idxDiv{D}\nabla^*)$ 
from any smooth distance $D(\cdot:\cdot)$ (called a divergence, and potentially asymmetric).
The {\em dual divergence} is defined by $D^*(\theta_1:\theta_2)=D(\theta_2:\theta_1)$. 
In particular, when the divergence is (i) a {\em Bregman divergence}~\cite{Bregman_1967}, we obtain an induced dually flat structure with   global dual affine coordinate systems (induced by the Legendre-Fenchel transformation of dual potential functions) and a dual Pythagorean theorem 
(\S\label{sec:igbd}), and (ii) a statistical $f$-divergence~\cite{Csiszar-1963} on a parametric family of probability distributions (the only separable divergence satisfying the information monotonicity property), we obtain the expected geometry~\cite{RefRepDuality-2015}, and its $\alpha$-extensions (\S\label{sec:if}).

In the second part (\S\ref{sec:AIG}), we illustrate these information-geometric structures with several applications:
We begin by considering the Bayesian hypothesis testing and show how Chernoff information 
can be characterized geometrically on the dually flat structure of an exponential family manifold.
We then show how to cluster statistical mixtures sharing the same component distributions on the dually flat mixture family manifold.

Finally, \S\ref{sec:concl} concludes this tutorial paper by summarizing important concepts of information geometry, and providing references  and textbooks~\cite{IG-2014,IG-2016} to more advanced structures and applications for further readings. 
We conclude by surveying recent advances of classes of distances from first principles.


